Efficient Contextual LLM Cascades through Budget-Constrained Policy Learning

Recent successes in natural language processing have led to the proliferation of large language models (LLMs) by multiple providers. Each LLM offering has different inference accuracy, monetary cost, and latency, and their accuracy further depends on the exact wording of the question (i.e., the specific prompt). At the same time, users often have a limit on monetary budget and latency to answer all their questions, and they do not know which LLMs to choose for each question to meet their accuracy and long term budget requirements. To navigate this rich design space, we propose TREACLE ($\underline{T}$hrifty $\underline{Rea}$soning via $\underline{C}$ontext-Aware $\underline{L}$LM and Prompt S$\underline{e}$lection), a reinforcement learning policy that jointly selects the model and prompting scheme while respecting the user's monetary cost and latency constraints. TREACLE uses the problem context, including question text embeddings (reflecting the type or difficulty of a query) and the response history (reflecting the consistency of previous responses) to make smart decisions. Our evaluations on standard reasoning datasets (GSM8K, CSQA, and LLC) with various LLMs and prompts show that TREACLE enables cost savings of up to 85% compared to baselines, while maintaining high accuracy. Importantly, it provides the user with the ability to gracefully trade off accuracy for cost.

==> sec/algo.tex <==
% \section{Cost and query-aware inference algorithms}
% We introduce online algorithms, denoted as $\alg$, designed to efficiently integrate multiple language models to answer a set of queries $\mathcal{Q}$ within the constraints of a given budget $B$. 
% % When a new query arises, our algorithm faces a critical decision: whether to return the current best answer or to initiate a re-query. Furthermore, it should determine the appropriate (model, prompt) pair $(\LM,P)$ to employ for this re-query.
% Recall that we have a list of language models $(\LM_i)_{i=1}^m$ along with corresponding prompt options $\{\LMPP_1,\LMPP_2,\ldots,\LMPP_i\}$. It is reasonable to assume that the model-prompt pairs are ordered (roughly) in ascending order of model capability and associated costs. When a new query arises, the algorithm's role is to select among three options based on the budget $B$: returning the current answer, re-querying with the existing model-prompt pair, or upgrading to a more powerful pair.

% To achieve this, we propose two methods: Consistency cascade or the implementation of a reinforcement learning model.
% \subsection{Consistency cascade algorithms:}
% The algorithm is shown in Alg.~\ref{alg:cascade}. $p_\text{low}$ and $p_\text{high}$ are 

% \begin{figure}[]
% \centering
% %\hspace{-35pt}
% \begin{subfigure}{}
%     \centering
% 	\begin{tikzpicture}
% 		\node at (0,0) [scale=0.4]{\includegraphics{img/Budget_p.pdf}};
% \end{tikzpicture}
% \end{subfigure}
% \vspace{-5pt}
% \caption{How does $p_\text{low}$ $p_\text{high}$ change with different budget.}\vspace{-10pt}
% \label{fig:Budget_p}
% \end{figure}
% \begin{figure}[]
% \centering
% %\hspace{-35pt}
% \begin{subfigure}{}
%     \centering
% 	\begin{tikzpicture}
% 		\node at (0,0) [scale=0.4]{\includegraphics{img/Budget_query.pdf}};
% \end{tikzpicture}
% \end{subfigure}
% \vspace{-5pt}
% \caption{How does $p_\text{low}$ $p_\text{high}$ change with different budget.}\vspace{-10pt}
% \label{fig:Budget_query}
% \end{figure}
% \begin{algorithm}[tb]
%    \caption{Consistency cascade}
%    \label{alg:cascade}
% \begin{algorithmic}
%    \STATE {\bfseries Input:} Query set $\mathcal{Q} = \{Q_1, Q_2, \ldots, Q_n\}$, Confidence predictor $f(\cdot)$, Model-Prompt pairs $\{\LMPP_1,\LMPP_2,\ldots,\LMPP_i\}$, The max query times for each Model-Prompt pairs $\text{MAX}_i$, Total budget $B$, Threshold $p_{\text{low}}$, $p_{\text{high}}$, Budget $B$
%    \STATE {\bfseries Output: Answers $\mathcal{Y}$} 
%     \STATE Initialize: Total cost $c=0$
%    \FOR{$i=1$ {\bfseries to} $n$}
%    \STATE Initialize: Answers $\hat{O}_{i} = []$, Model-Prompt pair index $j=1$, Query times for current Model-Prompt pairs $m=1$
%    \STATE Initialize $keepRequery = true$
%     \REPEAT 
%     \STATE $\hat{O}_{i} \leftarrow [\hat{O}_{i}, \LMPP_{j}(Q_{i})$]
%     \STATE $c = c+\text{cost}(\LMPP_{j}(Q_{i}))$
%     \IF{$f(Q_{i},\hat{O}_{i}) > p_{\text{high}}$}
%     \STATE $\hat{Y_i} = \LMPP_{j}(Q)$
%     \STATE $keepRequery = false$
%     \ELSIF {$f(Q_{i},\hat{O}_{i}) < p_{\text{low}}$ OR $m \geq $$\text{MAX}_j$}
%     \STATE $j=j+1$
%     \STATE $m = 0$
%     \ENDIF
%     \IF{$j = n$ and $m = \text{MAX}_j$}
%     \STATE $\hat{Y_i} = \text{majority}(\hat{O}_{i})$
%     \STATE $keepRequery = false$
%     \ENDIF
%     \UNTIL{$keepRequery == false$}
%     \IF{$c \geq B$}
%     \STATE break
%     \ENDIF
%    \ENDFOR
% \end{algorithmic}
% \end{algorithm}
% \input{sec/RL}

==> sec/calibration.tex <==
\section{Calibration for LLM Cascades}
Recall that we have a list of language models $(\text{LM}_i)_{i=1}^K$. We can assume these are (approximately) ordered by the increasing model capability and the respective costs. 


\vspace{-10pt}
\section{Twice can Suffice}
Suppose an LLM outputs a stochastic answer for a particular query with  distribution $\pb=[p_1~p_2~\dots~p_K]$. Let $p$ be the probability of the majority answer i.e.~$p=\arg\max_{i\in[K]}p_i$ and $q\leq p$ be the probability of the next most likely answer. $K$-stop self-consistency algorithm returns the majority answer when it occurs for the $K$'th time. 

\begin{theorem} Let $\alpha(\pb,K)$ be the probability that $K$-stop SC algorithm returns the true majority for distribution $\pb$. For any $\pb$, we have that \redp{are these true?}
\begin{enumerate}
\item $1-\alpha(\pb,2)\leq C(1-p)^2$ for some constant $C>0$. \redp{Implication: SC-2 improves accuracy by $O(1-p)$ whereas SC(3) and beyond will help at most $O(1-p^2)$}.
\item For any fixed $p$, as $\lim_{q\rightarrow 0}\alpha(\pb,2)=1$. \redp{Implication: SC-2 can in theory boost acc from a small p to 100\%.}
\item More generally, $\alpha(\pb,2)$ is lower and upper bounded as follows
\[
\text{lower??}(p,q)\leq \alpha(\pb,2)\leq\text{upper??}(p,q).
\]
\item \redp{This is optional} The relative benefit of SC-3 is upper bounded as follows
\[
\alpha(\pb,3)-\alpha(\pb,2)\leq\text{relative\_upper??}(p,q).
\]
\end{enumerate}
\end{theorem}

%\begin{theorem}[Stop at majority]
%\end{theorem}



==> sec/latency.tex <==
% \begin{figure}[]
% \centering
% %\hspace{-35pt}
%     \centering
% 	\begin{tikzpicture}
% 		\node at (0,0) [scale=0.25]{\includegraphics{img/Latency_Time.pdf}};
%   \node at (0,-1.55) [scale=0.8] {o'clock};
%   \node at (-2.15 ,0) [scale=0.8,rotate=90] {Latency (s)};
%   % \node at (0,-2) [scale=0.8] {50 times};
% \end{tikzpicture}
% \vspace{-7pt}
% \caption{End-to-end latency of querying LLM models over a 24-hour period.}\vspace{-13pt}
% \label{fig:Latency_Time}
% % \vspace{-0.1cm}
% \end{figure}

% \vspace{-0.4cm}
% \begin{table}[]
% \scriptsize
%     \centering
%     \scriptsize
%     \caption{Performance with time-varying API query latency.}
%     % \vspace{-10pt}
%      \label{tab:changing_latency}
%      \small
%      \scriptsize
%     \begin{tabular}{|p{1.4cm}|p{2cm}|p{2cm}|p{1.1cm}|}
% \hline
%    Method   & Accuracy with Time-varying Latency & Accuracy assuming Constant Latency    & Update time (s)\\ \hline
%   {\sf \scriptsize TREACLE}   & 86.4          &    76.1  & 0.02 \\ \hline
%   Calibrated  & \multirow{2}{*}{80.1}          &   \multirow{2}{*}{75.7} &  \multirow{2}{*}{617.30} \\ 
%   Cascade & & & \\\hline
%     \end{tabular}
%         % }
%         % \vspace{-20pt}
% \end{table}

% \vspace{-5pt}
% \xuechen{remove the whole subsubsection: Time-Varying API Query Latency}
% \subsubsection{Time-Varying API Query Latency}
% \label{sec:latency}
% %\xuechen{move to appendix? xuechen stop here}
% The latency of querying LLM APIs (such as OpenAI's GPT models) may vary over the short term time based on network congestion or LLM inference time. %with an updated cost estimate. 
% %\carlee{is this the estimate of the cost of each query?} \xuechen{No. We estimate the average re-query latency for each model-prompt pair. See table 2}
% %For example, in our experiments later in \cref{tab:changing_latency}, we update the estimated latency per query every hour.
% %To evaluate whether our methods can adapt to-varying latency, 
% To showcase this, we recorded traces of the API latency (including communication and communication latency) over a 24-hour period. The measurements are shown in \cref{fig:Latency_Time}. 
% %The latency for the locally run Llama models remains constant at 8 s per query for the smaller Llama model and 16 s for the larger Llama model. The latency for cloud-based GPT models fluctuates over time, with a variance of 3.13 s.
% %\textbf{Time-varying costs.} 
% %Costs may change over the long term (\eg from updated API prices) or the short term (\eg from network congestion to the servers of LLM providers).
% %We assume that users continue to use LLMs to answer questions during this period of time-varying latency.
% %To adapt to time-varying latency, 
% We also modified \alg and the experimental setup slightly.
% Each hour, \alg attempts to answer the entire GSM8K test set with a budget of \$0.6,
% %\jiasi{why this number? 0.6*24 = 14.4 = total budget for ``Constant Latency''?} \xuechen{Select a budget that \alg has clear improvement. With too low or too high a budget, almost all problems use gpt4, so there is only minor improvement. each hour has a budget separately. Couldn't use the budget for other hours. }
% using the historical average latency from the previous hour to update the per-query cost in the denominator of $\mathcal{B}_k$. The budget resets every hour.
% %To handle this, \alg periodically updates its estimate of the remaining budget $\mathcal{B}_k$ in the state vector.
% %Specifically, it periodically updates the denominator of $\mathcal{B}_k$ with the new  average per-query cost of $\LMPP_k$.
% We compare this to the vanilla \alg shown previously, which 
% %As a baseline, we assume that the algorithm 
% has the same total budget and
% uses a fixed latency in the denominator of $\mathcal{B}_k$ for the entire 24-h period; for example, for GPT models, it assumes a fixed average latency of 6 s.
% The results in \cref{tab:changing_latency} indicate that \alg that adapts to time-varying achieves higher accuracy than the version that assumes constant latency. The update time to calculate the new $\mathcal{B}_k$ each hour is also minimal, at 20 ms.
% %For $\alg$, we use $\mathcal{B_\text{remaining}} = \{\frac{\text{Total remaining budget}}{\text{Average cost per query for }\mathcal{\LMPP}}\}$ as the state, allowing us to update the "$\text{Average cost per query for }\mathcal{\LMPP}$" with real-time data quickly.
% %We also made simmilar modifications to \algU to incorporate time-varying latency.
% %We update the $p_{\text{low}}$ and $p_{\text{high}}$ parameters every hour \jiasi{right?}
% %based on the new cost for the Calibrated Cascade algorithm, 
% %based on the new latency values,
% %but this requires incorporating new latency values and
% %but this requires conducting a grid search on the validation set. This can be slow when the validation set is large, and contributes to the high update time in \cref{tab:changing_latency}.
% %, and using a smaller validation set may impact the performance. 
% %The results are displayed in Table ~\ref{tab:changing_latency}. They indicate that $\alg$ quickly adapts to new latency conditions.


==> sec/method.tex <==
\section{Can LLM evaluate the correctness of reasoning problems?}
\xuechen{Evaluate with ECE, correlation and F1 score}
\xuechen{System, confidence?}
An important aspect of this problem is estimating the performance of each model-prompt pairing employed for individual queries. A predictor function denoted as $f(\cdot)$, is formulated for performance estimation. This estimation assists in deciding whether to return the current response or to re-query and guides us to determine which model-prompt pairing to query next.

Straightforwardly, performance estimation can rely on both the question and the answer of the current query $O_i$, $i$ is the number of queries, represented as $f(Q, O_i)$, $i$ is the number of queries.

\textbf{LLM self-evaluation}: Firstly, we investigate whether LLMs can self-evaluate. After the model provides an answer, we inquire about its confidence level regarding the previous response, using the prompt "{Answer} is your previous answer to question {Query}, please rate your confidence in this answer on a scale of 0 to 10, where 0 signifies no confidence at all, and 10 signifies full confidence." We observe that LLMs are consistently over-confident. Additionally, this approach is quite costly, as it requires inputting all answers and queries, which entails a substantial number of tokens. \xuechen{TODO: @Ege, please edit the prompt}

\textbf{Text embedding}: We use text embeddings to predict the correctness of answers. For text, we experiment with using only the question and using both the question and answer simultaneously. We also try different encoders, including MiniBERT~\cite{turc2019well}, T5\cite{raffel2020exploring}, and the embedding model provided by OpenAI \xuechen{how to cite?}. We even attempte to fine-tune a DistilBERT~\cite{sanh2019distilbert} following frugalGPT~\cite{chen2023frugalgpt}. Then, we train a two-layer neural network to use these embeddings to predict answer correctness. We introduce the calibration technique to address potential accuracy reduction due to data imbalance. Among these approaches, using OpenAI's API along with a two-layer neural network and calibration yield the best results, although it still couldn't accurately predict. We include it as a baseline. 
\subsection{Evaluation with previous answers:\xuechen{@Xuechen todo}}
Evaluating the correctness of a reasoning question's answer solely based on its literal expression is highly challenging, as errors can be subtle even when the reasoning paths seem promising. Given the introduction of variability through different prompts and non-zero temperature values, we suggest that we can obtain a more accurate performance estimation by re-querying and cross-checking these answers. Therefore, the predictor is denoted as $f(Q, \{O_0, O_1, ..., O_i\})$.

\textbf{Consistency:} Some papers propose the use of consistency\cite{yue2023large,wang2022self}. We suggest that enhancing the variety in generating responses, for instance, by employing diverse model-prompt-temperature combinations, can accelerate decision-making with consistency, resulting in increased accuracy. This has the potential to reduce costs substantially. The results are shown in Table.~\ref{tab:consistency}. \xuechen{Should we add majority v.s. cascade?}


\begin{table*}[ht]
    \centering
    % \scriptsize
    \caption{\xuechen{fill in caption}}
    \begin{tabular}{c|cc|cc}
\hline
   \multirow{2}{*}{Model}   & \multicolumn{2}{c|}{GSM8K}             & \multicolumn{2}{c}{CSQA}               \\ \cline{2-5}  
 & \multicolumn{1}{c|}{Accuracy} & Price & \multicolumn{1}{c|}{Accuracy} & Price \\ \hline \hline
  Llama-2-13b-chat(T=0,CoT)+ GPT-3.5-turbo(T=0,CoT)   & \multicolumn{1}{c|}{}          &       & \multicolumn{1}{c|}{}          &       \\ \hline
      Llama-2-13b-chat(T=0,CoT)+GPT-3.5-turbo(T=0,CoT) +  GPT-3.5-turbo(T=1,CoT)& \multicolumn{1}{c|}{}          &       & \multicolumn{1}{c|}{}          &       \\ \hline
     GPT-3.5-turbo(T=0,``Math Solver'')   & \multicolumn{1}{c|}{}          &       & \multicolumn{1}{c|}{}          &       \\ \hline
   GPT-3.5-turbo(T=0,CoT)   & \multicolumn{1}{c|}{}          &       & \multicolumn{1}{c|}{}          &       \\ \hline
    \end{tabular}
        % }
    \label{tab:consistency}
\end{table*}


\input{sec/query-dependent uncertainty}
\input{sec/algo.tex}

==> sec/query-dependent_uncertainty.tex <==
%\textbf{Query-dependent uncertainty estimation:}

Finally, we take a deep dive into evaluating the learned $f$ function (from \algU), whose goal is to estimate the uncertainty of a given answer.
%We compare those uncertainty quantization methods and our Query-dependent uncertainty outperform other baselines. 
We compare our learned $f$ against several other uncertainty prediction methods: self-evaluation (\jiasi{explanation} \xuechen{in appendix}), text embedding (\jiasi{explanation}\xuechen{in appendix}), and \BMajority.
The results are shown in Table~\ref{tab:evaluation} in terms of the Expected Calibration Error (ECE) \jiasi{ref} \xuechen{\cite{naeini2015obtaining}} and F1-score.
Intuitively, ECE captures the difference between the predicted and true uncertainty, so a lower value is better.
\jiasi{isn't F1-score for classification? how are we using it for uncertainty prediction which is not classification? one sentence summary would be good here.} \xuechen{binary classification. Predict the answer is correct or not}
Our uncertainty predictor $f$ has the best performance for both metrics.
We also examine the performance for different budget sizes.
%When we perform a re-query, we not only obtain a new answer but also utilize this answer to enhance our assessment of the credibility and trustworthiness of our current response. \jiasi{why trustworthy and credible? This comes up suddenly}
The results are depicted in Fig.~\ref{fig:ece_query}. Regardless of the method employed, the ECE steadily decreases as the budget increases, because a larger budget allows for more re-queries and better uncertainty prediction.
% \textbf{Features:}

\begin{table}[ht]
    \centering
    \scriptsize
    \caption{\small{Comparing the uncertainty prediction methods.}}
    \begin{tabular}{c|cc|cc}
\hline
   \multirow{2}{*}{Method}   & \multicolumn{2}{c|}{GSM8K}             & \multicolumn{2}{c}{CSQA}               \\ \cline{2-5}  
 & \multicolumn{1}{c|}{ECE $\downarrow$} & F1-score $\uparrow$ & \multicolumn{1}{c|}{ECE $\downarrow$} & F1-score $\uparrow$\\ \hline \hline
      Self-evaluation & \multicolumn{1}{c|}{0.22}          &    0.63   & \multicolumn{1}{c|}{0.06}&    0.69   \\ \hline
     Text embedding   & \multicolumn{1}{c|}{0.15}         &     0.68   & \multicolumn{1}{c|}{0.24}          &   0.64    \\ \hline
   \BMajority  & \multicolumn{1}{c|}{0.10}          &    0.91   & \multicolumn{1}{c|}{0.17}          &    0.87   \\ \hline
      Uncertainty predictor $f$   & \multicolumn{1}{c|}{0.04}          &  0.96     & \multicolumn{1}{c|}{0.05}          &  0.90     \\ \hline
    \end{tabular}
        % }
    \label{tab:evaluation}
\end{table}

\begin{figure}[]
\centering
%\hspace{-35pt}
\begin{subfigure}[b]{0.23\textwidth}
    \centering
	\begin{tikzpicture}
		\node at (0,0) [scale=0.24]{\includegraphics{img/ece_2.pdf}};
  % \node at (0,-1.5) [scale=0.8] {ECE};
\end{tikzpicture}\label{fig:ece}
\end{subfigure}
\begin{subfigure}[b]{0.23\textwidth}
    \centering
	\begin{tikzpicture}
		\node at (0,0) [scale=0.24]{\includegraphics{img/f1_2.pdf}};
  % \node at (0,-1.5) [scale=0.8] {F1};
\end{tikzpicture}
\end{subfigure}
\vspace{-10pt}
\caption{\small{Estimate the performance for accuracy with increasing number of queries.}
%\jiasi{change ``consistency'' to \BMajority and ``Uncertainty prediction'' to ``Uncertainty predictor $f$''. Also bigger text please.} \xuechen{updated}
}\vspace{-10pt}
\label{fig:ece_query}
\end{figure}


==> sec/uncertainty.tex <==
\subsection{Uncertainty Quantification via \algU}
\label{sec:uncertainty}

\jiasi{skip this section for now, may remove due to space}
%An important part of our method is to estimate the performance of each model-prompt pair employed in individual queries.
A key intuition in \alg is that it should implicitly learn whether the response provided by the current model-prompt pair is accurate and use this to decide the optimal action.
This is represented by the ``response consistency'' feature in the state, as described earlier.
In this subsection, we delve deeper into this intuition and propose \algU, a variant of \alg that explicitly learns to estimate the response accuracy.
It includes a prediction function 
%A predictor function denoted as 
$f(\cdot)$
%, is designed for performance estimation, 
that helps decide whether to return the current response or to re-query, and also assists in determine which model-prompt pairing to query next. 
In other words, $f$ is learned implicitly in \alg, while it is explicitly learned in \algU.
%, it is explicitly learned. % by an external model. %, driving the Calibrated Cascade Algorithm. 

% Straightforwardly, performance estimation can rely on both the question and the answer of the current query $O_i$, $i$ is the number of queries, represented as $f(Q, O_i)$. We investigate that the performance can not be self-evaluated or predicted with text embedding.     

% \textbf{LLM self-evaluation}: Firstly, we investigate whether LLMs can self-evaluate. After the model provides an answer, we inquire about its confidence level regarding the previous response, using the prompt "{Answer} is your previous answer to question {Query}, please rate your confidence in this answer on a scale of 0 to 10, where 0 signifies no confidence at all, and 10 signifies full confidence." We observe that LLMs are consistently over-confident. Additionally, this approach is quite costly, as it requires inputting all answers and queries, which entails a substantial number of tokens. \xuechen{TODO: @Ege, please edit the prompt}

% \textbf{Text embedding}: We use text embeddings to predict the correctness of answers. For text, we experiment with using only the question and using both the question and answer simultaneously. We also try different encoders, including MiniBERT~\cite{turc2019well}, T5\cite{raffel2020exploring}, and the embedding model provided by OpenAI \xuechen{how to cite?}. We even attempte to fine-tune a DistilBERT~\cite{sanh2019distilbert} following frugalGPT~\cite{chen2023frugalgpt}. Then, we train a two-layer neural network to use these embeddings to predict answer correctness. We introduce the calibration technique to address potential accuracy reduction due to data imbalance. Among these approaches, using OpenAI's API along with a two-layer neural network and calibration yield the best results, although it still couldn't accurately predict. We include it as a baseline. 
% \subsection{Evaluation with previous answers:\xuechen{@Xuechen todo}}
In designing $f$, we observed that evaluating the correctness of a response solely based on a query-response pair $(Q_i, \hat{Y}_i)$ 
%\jiasi{$O$ or $O_i$?} \xuechen{$Y_i$}
is highly challenging in reasoning tasks, as errors can be subtle even when the reasoning paths seem to be promising. \jiasi{can you elaborate on ``errors can be subtle even when reasoning paths seem to be promising'' more?} \xuechen{Promising reasoning path doesn't mean the final answer could be correct. So, directly utilizing the text couldn't achieve accurate performance prediction.}
Inspired by previous works \cite{cai2023humanintheloop, yue2023large}, we incorporated wide range of features as inputs to a machine learning model to learn $f$, such as query trajectories and stationary statistics. 
\jiasi{integrate next sentence here, moved up from Experiments}
Some recent papers have introduced the concept of consistency \cite{yue2023large,wang2022self}. We propose that enhancing response diversity, for example, by leveraging various model-prompt-temperature combinations, can expedite decision-making with consistency, ultimately leading to improved accuracy.

Thus, given the introduction of variability through different prompts and non-zero temperature values \jiasi{what are you trying to say here? that re-querying helps us get better performance even with variable prompts?} \xuechen{re-querying with diverse answers helps. Re-query with the same prompts and zero temperature value will always achieve same answer so it won't help. We try to diversify the answers by deploying different prompts and non-zero temperature values}, we have a more accurate performance estimation by re-querying and accumulating the related query statistics. 
\jiasi{should we provide a full list of features used to learn $f$?} \xuechen{same as dqn}
Therefore, the predictor function maps question and the past answer statistics to $f(Q, \{O_0, O_1, ..., O_i\})$.    
            \jiasi{how can multiple $O$ be the inputs to $f$? Is it all the correct answers from previous queries? The output of $f$ is the confidence, correct? Need to say explicitly} \xuechen{multiple $O$: All previous response(if there have been re-queries)}


\jiasi{I think the previous paragraph needs to be re-written, it is kind of hard to understand. Is it trying to provide a high level overview of \algU? Or justifying certain design decisions like feature selection?}

% \textbf{Consistency:} Some papers propose the use of consistency\cite{yue2023large,wang2022self}. We suggest that enhancing the variety in generating responses, for instance, by employing diverse model-prompt-temperature combinations, can accelerate decision-making with consistency, resulting in increased accuracy. This has the potential to reduce costs substantially. The results are shown in Table.~\ref{tab:consistency}. \xuechen{Should we add majority v.s. cascade?}


% \begin{table*}[ht]
%     \centering
%     % \scriptsize
%     \caption{\xuechen{fill in caption}}
%     \begin{tabular}{c|cc|cc}
% \hline
%    \multirow{2}{*}{Model}   & \multicolumn{2}{c|}{GSM8K}             & \multicolumn{2}{c}{CSQA}               \\ \cline{2-5}  
%  & \multicolumn{1}{c|}{Accuracy} & Price & \multicolumn{1}{c|}{Accuracy} & Price \\ \hline \hline
%   Llama-2-13b-chat(T=0,CoT)+ GPT-3.5-turbo(T=0,CoT)   & \multicolumn{1}{c|}{}          &       & \multicolumn{1}{c|}{}          &       \\ \hline
%       Llama-2-13b-chat(T=0,CoT)+GPT-3.5-turbo(T=0,CoT) +  GPT-3.5-turbo(T=1,CoT)& \multicolumn{1}{c|}{}          &       & \multicolumn{1}{c|}{}          &       \\ \hline
%      GPT-3.5-turbo(T=0,``Math Solver'')   & \multicolumn{1}{c|}{}          &       & \multicolumn{1}{c|}{}          &       \\ \hline
%    GPT-3.5-turbo(T=0,CoT)   & \multicolumn{1}{c|}{}          &       & \multicolumn{1}{c|}{}          &       \\ \hline
%     \end{tabular}
%         % }
%     \label{tab:consistency}
% \end{table*}


% \input{sec/query-dependent uncertainty}
% \input{sec/algo.tex}
%\subsection{Calibrated Cascade Algorithm}
\textbf{Algorithm overview.} %Our uncertainty quantification model is the main component of Calibrated Cascade Algorithm, which can be viewed as the hard-coded version of $\alg$.
Given a learned $f$, \algU utilizes it directly in determining its next action.
%Predicted uncertainty is utilized directly in determining the next action. 
If $f$ estimates high confidence in the LLM's response (above a threshold $p_\text{high}$), the response is directly returned.
%the model is confident in its answer, we directly return it. 
Otherwise,
%if uncertainty persists, 
we initiate a re-query.
If so, we the same model-prompt pair may be used (if the confidence is greater than a threshold $p_\text{low}$) or the next model-prompt pair in the sorted list (if the confidence is lower than $p_\text{low}$).
%with the choice of model-prompt pair for re-query also being decided by the estimated uncertainty.
\cref{alg:cascade} provides full details.

% \begin{figure}[]
% \centering
% %\hspace{-35pt}
% \begin{subfigure}{}
%     \centering
% 	\begin{tikzpicture}
% 		\node at (0,0) [scale=0.4]{\includegraphics{img/Budget_p.pdf}};
% \end{tikzpicture}
% \end{subfigure}
% \vspace{-5pt}
% \caption{How does $p_\text{low}$ $p_\text{high}$ change with different budget.}\vspace{-10pt}
% \label{fig:Budget_p}
% \end{figure}
% \begin{figure}[]
% \centering
% %\hspace{-35pt}
% \begin{subfigure}{}
%     \centering
% 	\begin{tikzpicture}
% 		\node at (0,0) [scale=0.4]{\includegraphics{img/Budget_query.pdf}};
% \end{tikzpicture}
% \end{subfigure}
% \vspace{-5pt}
% \caption{How does $p_\text{low}$ $p_\text{high}$ change with different budget.}\vspace{-10pt}
% \label{fig:Budget_query}
% \end{figure}
% \begin{algorithm}[tb]
%    \caption{Consistency cascade}
%    \label{alg:cascade}
% \begin{algorithmic}
%    \STATE {\bfseries Input:} Query set $\mathcal{Q} = \{Q_1, Q_2, \ldots, Q_n\}$, Confidence predictor $f(\cdot)$, Model-Prompt pairs $\{\LMPP_1,\LMPP_2,\ldots,\LMPP_i\}$, The max query times for each Model-Prompt pairs $\text{MAX}_i$, Total budget $B$, Threshold $p_{\text{low}}$, $p_{\text{high}}$, Budget $B$
%    \STATE {\bfseries Output: Answers $\mathcal{Y}$} 
%     \STATE Initialize: Total cost $c=0$
%    \FOR{$i=1$ {\bfseries to} $n$}
%    \STATE Initialize: Answers $\hat{O}_{i} = []$, Model-Prompt pair index $j=1$, Query times for current Model-Prompt pairs $m=1$
%    \STATE Initialize $keepRequery = true$
%     \REPEAT 
%     \STATE $\hat{O}_{i} \leftarrow [\hat{O}_{i}, \LMPP_{j}(Q_{i})$]
%     \STATE $c = c+\text{cost}(\LMPP_{j}(Q_{i}))$
%     \IF{$f(Q_{i},\hat{O}_{i}) > p_{\text{high}}$}
%     \STATE $\hat{Y_i} = \LMPP_{j}(Q)$
%     \STATE $keepRequery = false$
%     \ELSIF {$f(Q_{i},\hat{O}_{i}) < p_{\text{low}}$ OR $m \geq $$\text{MAX}_j$}
%     \STATE $j=j+1$
%     \STATE $m = 0$
%     \ENDIF
%     \IF{$j = n$ and $m = \text{MAX}_j$}
%     \STATE $\hat{Y_i} = \text{majority}(\hat{O}_{i})$
%     \STATE $keepRequery = false$
%     \ENDIF
%     \UNTIL{$keepRequery == false$}
%     \IF{$c \geq B$}
%     \STATE break
%     \ENDIF
%    \ENDFOR
% \end{algorithmic}
% \end{algorithm}
